Can We Use SE-specific Sentiment Analysis Tools in a Cross-Platform Setting?

In this paper, we address the problem of using sentiment analysis tools 'off-the-shelf,' that is when a gold standard is not available for retraining. We evaluate the performance of four SE-specific tools in a cross-platform setting, i.e., on a test set collected from data sources different from the one used for training. We find that (i) the lexicon-based tools outperform the supervised approaches retrained in a cross-platform setting and (ii) retraining can be beneficial in within-platform settings in the presence of robust gold standard datasets, even using a minimal training set. Based on our empirical findings, we derive guidelines for reliable use of sentiment analysis tools in software engineering.

==> big_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\begin{tabular}{cccllllllllllllllll}
\multirow{2}{*}{\textbf{Setting}} & \multirow{2}{*}{\textbf{Test set}} & \multirow{2}{*}{\textbf{Training set}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Class}}} & \multicolumn{3}{c}{\textbf{Senti4SD}} & \multicolumn{3}{c}{\textbf{Senti4SD (no BoW)}} & \multicolumn{3}{c}{\textbf{SentiCR}} & \multicolumn{3}{c}{\textbf{SentiStrength-SE}} & \multicolumn{3}{c}{\textbf{DEVA}} \\
 &  &  & \multicolumn{1}{c}{} & \multicolumn{1}{c}{\textit{P}} & \multicolumn{1}{c}{\textit{R}} & \multicolumn{1}{c}{\textit{F1}} & \multicolumn{1}{c}{\textit{P}} & \multicolumn{1}{c}{\textit{R}} & \multicolumn{1}{c}{\textit{F1}} & \multicolumn{1}{c}{\textit{P}} & \multicolumn{1}{c}{\textit{R}} & \multicolumn{1}{c}{\textit{F1}} & \multicolumn{1}{c}{\textit{P}} & \multicolumn{1}{c}{\textit{R}} & \multicolumn{1}{c}{\textit{F1}} & \multicolumn{1}{c}{\textit{P}} & \multicolumn{1}{c}{\textit{R}} & \multicolumn{1}{c}{\textit{F1}} \\
\multirow{5}{*}{Within-platform} & \multirow{5}{*}{GitHub} & \multirow{5}{*}{GitHub} & Negative & \multicolumn{1}{c}{0.92} & \multicolumn{1}{c}{0.90} & \multicolumn{1}{c}{0.91} & \multicolumn{3}{c}{\multirow{5}{*}{--}} & \multicolumn{1}{c}{0.90} & \multicolumn{1}{c}{0.63} & \multicolumn{1}{c}{0.74} & \multicolumn{1}{c}{0.79} & \multicolumn{1}{c}{0.77} & \multicolumn{1}{c}{0.78} & \multicolumn{1}{c}{0.65} & \multicolumn{1}{c}{0.68} & \multicolumn{1}{c}{0.67} \\
 &  &  & Neutral & \multicolumn{1}{c}{0.90} & \multicolumn{1}{c}{0.93} & \multicolumn{1}{c}{0.92} & \multicolumn{3}{c}{} & \multicolumn{1}{c}{0.76} & \multicolumn{1}{c}{0.94} & \multicolumn{1}{c}{0.84} & \multicolumn{1}{c}{0.78} & \multicolumn{1}{c}{0.86} & \multicolumn{1}{c}{0.82} & \multicolumn{1}{c}{0.83} & \multicolumn{1}{c}{0.71} & \multicolumn{1}{c}{0.77} \\
 &  &  & Positive & \multicolumn{1}{c}{0.95} & \multicolumn{1}{c}{0.91} & \multicolumn{1}{c}{0.93} & \multicolumn{3}{c}{} & \multicolumn{1}{c}{0.89} & \multicolumn{1}{c}{0.85} & \multicolumn{1}{c}{0.87} & \multicolumn{1}{c}{0.86} & \multicolumn{1}{c}{0.76} & \multicolumn{1}{c}{0.81} & \multicolumn{1}{c}{0.69} & \multicolumn{1}{c}{0.81} & \multicolumn{1}{c}{0.75} \\
 &  &  & \textit{Micro-avg.} & \multicolumn{1}{c}{\textit{0.92}} & \multicolumn{1}{c}{\textit{0.92}} & \multicolumn{1}{c}{\textit{0.92}} & \multicolumn{3}{c}{} & \multicolumn{1}{c}{\textit{0.82}} & \multicolumn{1}{c}{\textit{0.82}} & \multicolumn{1}{c}{\textit{0.82}} & \multicolumn{1}{c}{\textit{0.80}} & \multicolumn{1}{c}{\textit{0.80}} & \multicolumn{1}{c}{\textit{0.80}} & \multicolumn{1}{c}{\textit{0.73}} & \multicolumn{1}{c}{\textit{0.73}} & \multicolumn{1}{c}{\textit{0.73}} \\
 &  &  & \textit{Macro-avg.} & \multicolumn{1}{c}{\textit{0.92}} & \multicolumn{1}{c}{\textit{0.92}} & \multicolumn{1}{c}{\textit{0.92}} & \multicolumn{3}{c}{} & \multicolumn{1}{c}{\textit{0.85}} & \multicolumn{1}{c}{\textit{0.81}} & \multicolumn{1}{c}{\textit{0.82}} & \multicolumn{1}{c}{\textit{0.81}} & \multicolumn{1}{c}{\textit{0.80}} & \multicolumn{1}{c}{\textit{0.80}} & \multicolumn{1}{c}{\textit{0.72}} & \multicolumn{1}{c}{\textit{0.73}} & \multicolumn{1}{c}{\textit{0.73}} \\
\multirow{5}{*}{Cross-platform} & \multirow{5}{*}{GitHub} & \multirow{5}{*}{Stack Overflow} & Negative & \textbf{0.79} & 0.5 & 0.61 & 0.75 & \textbf{0.83} & \textbf{0.79} & 0.78 & 0.34 & 0.47 & 0.79 & 0.77 & 0.78 & 0.65 & 0.68 & 0.67 \\
 &  &  & Neutral & 0.71 & 0.85 & 0.77 & 0.82 & 0.78 & 0.80 & 0.6 & \textbf{0.93} & 0.73 & 0.78 & 0.86 & \textbf{0.82} & \textbf{0.83} & 0.71 & 0.77 \\
 &  &  & Positive & 0.76 & 0.84 & 0.80 & \textbf{0.88} & \textbf{0.85} & \textbf{0.86} & 0.86 & 0.67 & 0.75 & 0.86 & 0.76 & 0.81 & 0.69 & 0.81 & 0.75 \\
 &  &  & \textit{Micro-avg.} & \textit{0.74} & \textit{0.74} & \textit{0.74} & \textit{\textbf{0.82}} & \textit{\textbf{0.82}} & \textit{\textbf{0.82}} & \textit{0.68} & \textit{0.68} & \textit{0.68} & \textit{0.8} & \textit{0.8} & \textit{0.8} & \textit{0.73} & \textit{0.73} & \textit{0.73} \\
 &  &  & \textit{Macro-avg.} & \textit{0.76} & \textit{\textbf{0.84}} & \textit{0.80} & \textit{\textbf{0.82}} & \textit{0.82} & \textit{\textbf{0.82}} & \textit{0.75} & \textit{0.65} & \textit{0.65} & \textit{0.81} & \textit{0.8} & \textit{0.8} & \textit{0.72} & \textit{0.73} & \textit{0.73} \\
\multicolumn{3}{r}{\multirow{2}{*}{\textit{Differences with the within-platform setting}}} & \textit{Micro-avg.} & \textit{-0.18} & \textit{-0.18} & \textit{-0.18} & \multicolumn{1}{c}{--} &  &  & \textit{-0.14} & \textit{-0.14} & \textit{-0.14} & \multicolumn{3}{c}{\multirow{2}{*}{--}} & \multicolumn{3}{c}{\multirow{2}{*}{--}} \\
\multicolumn{3}{r}{} & \textit{Macro-avg.} & \textit{-0.16} & \textit{-0.08} & \textit{-0.12} &  &  &  & \textit{-0.10} & \textit{-0.16} & \textit{-0.17} & \multicolumn{3}{c}{} & \multicolumn{3}{c}{} \\
\multirow{5}{*}{Cross-platform} & \multirow{5}{*}{GitHub} & \multirow{5}{*}{Jira} & Negative & 0.84 & 0.51 & 0.63 & \textbf{0.86} & 0.5 & 0.64 & 0.84 & 0.24 & 0.37 & 0.79 & \textbf{0.77} & \textbf{0.78} & 0.65 & 0.68 & 0.67 \\
 &  &  & Neutral & 0.59 & 0.96 & 0.73 & 0.62 & 0.95 & 0.75 & 0.51 & \textbf{0.98} & 0.67 & 0.78 & 0.86 & 0.82 & 0.83 & 0.71 & 0.77 \\
 &  &  & Positive & \textbf{0.93} & 0.45 & 0.61 & 0.91 & 0.57 & 0.7 & 0.92 & 0.35 & 0.51 & 0.86 & 0.76 & \textbf{0.81} & 0.69 & \textbf{0.81} & 0.75 \\
 &  &  & \textit{Micro-avg.} & \textit{0.68} & \textit{0.68} & \textit{0.68} & \textit{0.71} & \textit{0.71} & \textit{0.71} & \textit{0.58} & \textit{0.58} & \textit{0.58} & \textit{\textbf{0.80}} & \textit{\textbf{0.80}} & \textit{\textbf{0.80}} & \textit{0.73} & \textit{0.73} & \textit{0.73} \\
 &  &  & \textit{Macro-avg.} & \textit{0.79} & \textit{0.64} & \textit{0.66} & \textit{0.79} & \textit{0.67} & \textit{0.69} & \textit{0.76} & \textit{0.52} & \textit{0.52} & \textit{\textbf{0.81}} & \textit{\textbf{0.80}} & \textit{\textbf{0.80}} & \textit{0.72} & \textit{0.73} & \textit{0.73} \\
\multicolumn{3}{r}{\multirow{2}{*}{\textit{Differences with the within-platform setting}}} & \textit{Micro-avg.} & \textit{-0.24} & \textit{-0.24} & \textit{-0.24} & \multicolumn{1}{c}{\textit{--}} & \textit{} & \textit{} & \textit{-0.24} & \textit{-0.24} & \textit{-0.24} & \multicolumn{3}{c}{\multirow{2}{*}{\textit{--}}} & \multicolumn{3}{c}{\multirow{2}{*}{\textit{--}}} \\
\multicolumn{3}{r}{} & \textit{Macro-avg.} & \textit{-0.13} & \textit{-28} & \textit{-0.26} & \textit{} & \textit{} & \textit{} & \textit{-0.09} & \textit{-0.29} & \textit{-0.3} & \multicolumn{3}{c}{} & \multicolumn{3}{c}{} \\
\multirow{5}{*}{Within-platform} & \multirow{5}{*}{Stack Overflow} & \multirow{5}{*}{Stack Overflow} & Negative & 0.81 & 0.87 & 0.84 & \multicolumn{3}{c}{\multirow{3}{*}{--}} & 0.79 & 0.74 & 0.76 & 0.74 & 0.79 & 0.76 & 0.67 & 0.79 & 0.73 \\
 &  &  & Neutral & 0.86 & 0.81 & 0.84 & \multicolumn{3}{c}{} & 0.8 & 0.82 & 0.81 & 0.76 & 0.76 & 0.76 & 0.84 & 0.68 & 0.75 \\
 &  &  & Positive & 0.91 & 0.92 & 0.92 & \multicolumn{3}{c}{} & 0.88 & 0.9 & 0.89 & 0.89 & 0.84 & 0.86 & 0.85 & 0.9 & 0.87 \\
 &  &  & \textit{Micro-avg.} & \textit{0.87} & \textit{0.87} & \textit{0.87} & \multicolumn{3}{c}{\multirow{2}{*}{--}} & \textit{0.83} & \textit{0.83} & \textit{0.83} & \textit{0.8} & \textit{0.8} & \textit{0.8} & \textit{0.79} & \textit{0.79} & \textit{0.79} \\
 &  &  & \textit{Macro-avg.} & \textit{0.86} & \textit{0.87} & \textit{0.87} & \multicolumn{3}{c}{} & \textit{0.82} & \textit{0.82} & \textit{0.82} & \textit{0.8} & \textit{0.8} & \textit{0.79} & \textit{0.79} & \textit{0.79} & \textit{0.78} \\
\multirow{5}{*}{Cross-platform} & \multirow{5}{*}{Stack Overflow} & \multirow{5}{*}{GitHub} & Negative & 0.71 & 0.72 & 0.72 & 0.71 & \textbf{0.80} & 0.75 & 0.72 & 0.41 & 0.52 & 0.74 & 0.79 & 0.76 & 0.67 & 0.79 & 0.73 \\
 &  &  & Neutral & 0.71 & 0.8 & 0.75 & 0.79 & 0.75 & \textbf{0.77} & 0.64 & \textbf{0.88} & \textbf{0.74} & 0.76 & \textbf{0.76} & 0.76 & \textbf{0.84} & 0.68 & 0.75 \\
 &  &  & Positive & \textbf{0.92} & 0.78 & 0.84 & 0.9 & 0.85 & \textbf{0.87} & 0.84 & 0.78 & 0.81 & 0.89 & 0.84 & 0.86 & 0.85 & \textbf{0.90} & \textbf{0.87} \\
 &  &  & \textit{Micro-avg.} & \textit{0.77} & \textit{0.77} & \textit{0.77} & \textit{\textbf{0.80}} & \textit{\textbf{0.80}} & \textit{\textbf{0.80}} & \textit{0.72} & \textit{0.72} & \textit{0.72} & \textit{\textbf{0.80}} & \textit{\textbf{0.80}} & \textit{\textbf{0.80}} & \textit{0.79} & \textit{0.79} & \textit{0.79} \\
 &  &  & \textit{Macro-avg.} & \textit{0.78} & \textit{0.77} & \textit{0.77} & \textit{\textbf{0.80}} & \textit{\textbf{0.80}} & \textit{\textbf{0.80}} & \textit{0.73} & \textit{0.69} & \textit{0.69} & \textit{\textbf{0.80}} & \textit{\textbf{0.80}} & \textit{0.79} & \textit{0.79} & \textit{0.79} & \textit{0.78} \\
\multicolumn{3}{r}{\multirow{2}{*}{\textit{Differences with the within-platform setting}}} & \textit{Micro-avg.} & \textit{-0.10} & \textit{-0.10} & \textit{-0.10} & \textit{} & \textit{} & \textit{} & \textit{-0.11} & \textit{-0.11} & \textit{-0.11} & \multicolumn{3}{l}{\multirow{2}{*}{\textit{--}}} & \multicolumn{3}{l}{\multirow{2}{*}{\textit{--}}} \\
\multicolumn{3}{r}{} & \textit{Macro-avg.} & \textit{-0.09} & \textit{-0.10} & \textit{-0.10} & \textit{} & \textit{} & \textit{} & \textit{-0.09} & \textit{-0.13} & \textit{-0.13} & \multicolumn{3}{l}{} & \multicolumn{3}{l}{} \\
\multirow{5}{*}{Cross-platform} & \multirow{5}{*}{Stack Overflow} & \multirow{5}{*}{Jira} & Negative & 0.77 & 0.34 & 0.48 & \textbf{0.79} & 0.32 & 0.46 & 0.71 & 0.13 & 0.22 & 0.74 & \textbf{0.79} & \textbf{0.76} & 0.67 & \textbf{0.79} & 0.73 \\
 &  &  & Neutral & 0.56 & 0.93 & 0.70 & 0.57 & 0.93 & 0.70 & 0.46 & \textbf{0.97} & 0.62 & 0.76 & 0.76 & \textbf{0.76} & \textbf{0.84} & 0.68 & 0.75 \\
 &  &  & Positive & \textbf{0.96} & 0.65 & 0.78 & 0.92 & 0.70 & 0.79 & \textbf{0.96} & 0.38 & 0.54 & 0.89 & 0.84 & 0.86 & 0.85 & \textbf{0.90} & \textbf{0.87} \\
 &  &  & Micro-avg. & 0.68 & 0.68 & 0.68 & 0.68 & 0.68 & 0.68 & 0.54 & 0.54 & 0.54 & 0.80 & 0.80 & 0.80 & 0.79 & 0.79 & 0.79 \\
 &  &  & Macro-avg. & 0.76 & 0.64 & 0.65 & 0.76 & 0.65 & 0.65 & 0.71 & 0.49 & 0.46 & 0.80 & 0.80 & 0.79 & 0.79 & 0.79 & 0.78 \\
\multicolumn{3}{r}{\multirow{2}{*}{\textit{Differences with the within-platform setting}}} & \textit{Micro-avg.} & \textit{-0.19} & \textit{-0.19} & \textit{-0.19} & \textit{--} & \textit{} & \textit{} & \textit{-0.29} & \textit{-0.29} & \textit{-0.29} & \multicolumn{3}{l}{\multirow{2}{*}{\textit{--}}} & \multicolumn{3}{l}{\multirow{2}{*}{\textit{--}}} \\
\multicolumn{3}{r}{} & \textit{Macro-avg.} & \textit{-0.1} & \textit{-0.23} & \textit{-0.22} & \textit{} & \textit{} & \textit{} & \textit{-0.11} & \textit{-0.33} & \textit{-0.36} & \multicolumn{3}{l}{} & \multicolumn{3}{l}{} \\
\multirow{5}{*}{Within-platform} & \multirow{5}{*}{Jira} & \multirow{5}{*}{Jira} & Negative & 0.75 & 0.6 & 0.67 & \multicolumn{3}{c}{\multirow{3}{*}{--}} & 0.83 & 0.63 & 0.72 & 0.64 & 0.72 & 0.68 & 0.52 & 0.69 & 0.59 \\
 &  &  & Neutral & 0.87 & 0.89 & 0.88 & \multicolumn{3}{c}{} & 0.88 & 0.91 & 0.89 & 0.93 & 0.81 & 0.87 & 0.96 & 0.75 & 0.83 \\
 &  &  & Positive & 0.76 & 0.78 & 0.77 & \multicolumn{3}{c}{} & 0.79 & 0.81 & 0.8 & 0.69 & 0.93 & 0.79 & 0.63 & 0.9 & 0.74 \\
 &  &  & \textit{Micro-avg.} & \textit{0.83} & \textit{0.83} & \textit{0.83} & \textit{} & \textit{} & \textit{} & \textit{0.86} & \textit{0.86} & \textit{0.86} & \textit{0.82} & \textit{0.82} & \textit{0.82} & \textit{0.77} & \textit{0.77} & \textit{0.77} \\
 &  &  & \textit{Macro-avg.} & \textit{0.79} & \textit{0.76} & \textit{0.77} & \textit{} & \textit{} & \textit{} & \textit{0.83} & \textit{0.78} & \textit{0.8} & \textit{0.75} & \textit{0.82} & \textit{0.78} & \textit{0.69} & \textit{0.78} & \textit{0.72} \\
\multicolumn{1}{l}{\multirow{5}{*}{Cross-platform}} & \multicolumn{1}{l}{\multirow{5}{*}{Jira}} & \multicolumn{1}{l}{\multirow{5}{*}{GitHub}} & Negative & 0.57 & 0.64 & 0.61 & 0.57 & 0.61 & 0.59 & 0.75 & 0.56 & 0.64 & 0.64 & 0.72 & 0.68 & 0.52 & 0.69 & 0.59 \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & Neutral & 0.89 & 0.79 & 0.84 & 0.88 & 0.8 & 0.84 & 0.9 & 0.87 & 0.88 & 0.93 & 0.81 & 0.87 & 0.96 & 0.75 & 0.83 \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & Positive & 0.65 & 0.85 & 0.74 & 0.65 & 0.81 & 0.72 & 0.71 & 0.91 & 0.8 & 0.69 & 0.93 & 0.79 & 0.63 & 0.9 & 0.74 \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \textit{Micro-avg.} & \textit{0.78} & \textit{0.78} & \textit{0.78} & \textit{0.78} & \textit{0.78} & \textit{0.78} & \textit{0.84} & \textit{0.84} & \textit{0.84} & \textit{0.82} & \textit{0.82} & \textit{0.82} & \textit{0.77} & \textit{0.77} & \textit{0.77} \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \textit{Macro-avg.} & \textit{0.7} & \textit{0.76} & \textit{0.73} & \textit{0.70} & \textit{0.74} & \textit{0.71} & \textit{0.79} & \textit{0.78} & \textit{0.77} & \textit{0.75} & \textit{0.82} & \textit{0.78} & \textit{0.69} & \textit{0.78} & \textit{0.72} \\
\multicolumn{3}{r}{\multirow{2}{*}{\textit{Difference with the within-platform setting}}} & \textit{Micro-avg.} & \textit{-0.05} & \textit{-0.05} & \textit{-0.05} & \textit{--} & \textit{} & \textit{} & \textit{-0.7} & \textit{-0.7} & \textit{-0.7} & \multicolumn{3}{l}{\multirow{2}{*}{\textit{--}}} & \multicolumn{3}{l}{\multirow{2}{*}{\textit{--}}} \\
\multicolumn{3}{r}{} & \textit{Macro-avg.} & \textit{-0.09} & \textit{0} & \textit{-0.04} & \textit{} & \textit{} & \textit{} & \textit{-0.04} & \textit{0} & \textit{-0.03} & \multicolumn{3}{l}{} & \multicolumn{3}{l}{} \\
\multicolumn{1}{l}{\multirow{5}{*}{Cross-platform}} & \multicolumn{1}{l}{\multirow{5}{*}{Jira}} & \multicolumn{1}{l}{\multirow{5}{*}{Stack Overflow}} & Negative & 0.44 & 0.26 & 0.33 & 0.5 & 0.69 & 0.58 & 0.16 & 0.03 & 0.05 & 0.64 & 0.72 & 0.68 & 0.52 & 0.69 & 0.59 \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & Neutral & 0.83 & 0.79 & 0.81 & 0.92 & 0.73 & 0.81 & 0.75 & 0.94 & 0.83 & 0.93 & 0.81 & 0.87 & 0.96 & 0.75 & 0.83 \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & Positive & 0.57 & 0.85 & 0.68 & 0.63 & 0.9 & 0.74 & 0.72 & 0.49 & 0.58 & 0.69 & 0.93 & 0.79 & 0.63 & 0.9 & 0.74 \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \textit{Micro-avg.} & \textit{0.73} & \textit{0.73} & \textit{0.73} & \textit{0.76} & \textit{0.76} & \textit{0.76} & \textit{0.73} & \textit{0.73} & \textit{0.73} & \textit{0.82} & \textit{0.82} & \textit{0.82} & \textit{0.77} & \textit{0.77} & \textit{0.77} \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \textit{Macro-avg.} & \textit{0.62} & \textit{0.63} & \textit{0.61} & \textit{0.68} & \textit{0.78} & \textit{0.71} & \textit{0.54} & \textit{0.49} & \textit{0.49} & \textit{0.75} & \textit{0.82} & \textit{0.78} & \textit{0.69} & \textit{0.78} & \textit{0.72} \\
\multicolumn{3}{r}{\multirow{2}{*}{\textit{Differences with the within-platform setting}}} & \textit{Micro-avg.} & \textit{-0.1} & \textit{-0.1} & \textit{-0.1} & \textit{--} & \textit{} & \textit{} & \textit{-0.13} & \textit{-0.13} & \textit{-0.13} & \multicolumn{3}{l}{\multirow{2}{*}{--}} & \multicolumn{3}{l}{\multirow{2}{*}{--}} \\
\multicolumn{3}{r}{} & \textit{Macro-avg.} & \textit{-0.17} & \textit{-0.13} & \textit{-0.16} & \textit{} & \textit{} & \textit{} & \textit{-0.29} & \textit{-0.29} & \textit{-0.31} & \multicolumn{3}{l}{} & \multicolumn{3}{l}{}
\end{tabular}
\end{table*}

==> study-design.tex <==
In this section, we first describe the manually annotated datasets used for the performance assessment, and then the experimental setting of the current study following the benchmarking study ~\cite{Novielli18}, which we use as a reference for discussing our findings in Section~\ref{sec:discussion}.


%\subsection{Annotated Datasets}
%\label{sec:datasets}
%\input{datasets.tex}

%\subsection{Study Design}
%\label{sec:experimental-setting}
%\input{experimental-setting.tex}


==> tabellaok.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[h!]
\caption{Performance of SE-specific sentiment analysis tools in the cross-platform setting. For each setting, we highlight the best values for each metric in bold and the overall performance in Italic. The within-platform setting is reported in gray.}
\label{tab:results}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccl|lll|lll|lll|lll|lll}
\hline
\multirow{2}{*}{\textbf{Setting}} & \multirow{2}{*}{\textbf{Train set}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Polarity\\ Class\end{tabular}}}} & \multicolumn{3}{c}{\textbf{Senti4SD}} & \multicolumn{3}{c}{\textbf{Senti4SD (no BoW)}} & \multicolumn{3}{c}{\textbf{SentiCR}} & \multicolumn{3}{c}{\textbf{SentiStrength-SE}} & \multicolumn{3}{c}{\textbf{DEVA}} \\ \cline{4-18} 
 &  & \multicolumn{1}{c}{} & \multicolumn{1}{c}{\textit{P}} & \multicolumn{1}{c}{\textit{R}} & \multicolumn{1}{c}{\textit{F1}} & \multicolumn{1}{c}{\textit{P}} & \multicolumn{1}{c}{\textit{R}} & \multicolumn{1}{c}{\textit{F1}} & \multicolumn{1}{c}{\textit{P}} & \multicolumn{1}{c}{\textit{R}} & \multicolumn{1}{c}{\textit{F1}} & \multicolumn{1}{c}{\textit{P}} & \multicolumn{1}{c}{\textit{R}} & \multicolumn{1}{c}{\textit{F1}} & \multicolumn{1}{c}{\textit{P}} & \multicolumn{1}{c}{\textit{R}} & \multicolumn{1}{c}{\textit{F1}} \\ \hline
\multicolumn{18}{|c|}{\textit{Test set: GitHub}} \\ \hline
%\rowcolor{lightgray}
%\rowcolor[HTML]{EFEFEF} 
%\rowcolor{gray!10}
\multirow{5}{*}{Within-platform} & \multirow{5}{*}{GitHub} & Negative &.92 & .90 & .91 & \multicolumn{3}{c}{\multirow{5}{*}{--}} & .90 & .63 & .74 & .79 & .77 & .78 & .65 & .68 & .67 \\
%\rowcolor[HTML]{EFEFEF} 
 &  & Neutral & .90 & .93 & .92 & \multicolumn{3}{c}{} & .76 & .94 & .84 & .78 & .86 & .82 & .83 & .71 & .77 \\
%\rowcolor[HTML]{EFEFEF} 
 &  & Positive & .95 & .91 & .93 & \multicolumn{3}{c}{} & .89 & .85 & .87 &.86 & .76 & .81 & .69 & .81 & .75 \\
%\rowcolor[HTML]{EFEFEF} 
 &  & \textit{Micro-avg.} & \textit{.92} & \textit{.92} & \textit{.92} & \multicolumn{3}{c}{} & \textit{.82} & \textit{.82} & \textit{.82} & \textit{.80} & \textit{.80} & \textit{.80} & \textit{.73} & \textit{.73} & \textit{.73}\\
%\rowcolor[HTML]{EFEFEF} 
 &  & \textit{Macro-avg.} & \textit{.92} & \textit{.92} & \textit{.92} & \multicolumn{3}{c}{} & \textit{.85} & \textit{.81} & \textit{.82} & \textit{.81} & \textit{.80} & \textit{.80} & \textit{.72} & \textit{.73} & \textit{.73} \\
\hline
\multirow{5}{*}{Cross-platform} & \multirow{5}{*}{Stack Overflow} & Negative & \textbf{.79} & .50 & .61 & .75 & \textbf{.83} & \textbf{.79} & .78 & .34 & .47 & .79 & .77 & .78 & .65 & .68 & .67 \\
 &  & Neutral & .71 & .85 & .77 & .82 & .78 & .80 & .60 & \textbf{.93} & .73 & .78 & .86 & \textbf{.82} & \textbf{.83} & .71 & .77 \\
 &  & Positive & .76 & .84 & .80 & \textbf{.88} & \textbf{.85} & \textbf{.86} & .86 & .67 & .75 & .86 & .76 & .81 & .69 & .81 & .75 \\
 &  & \textit{Micro-avg.} & \textit{.74} & \textit{.74} & \textit{.74} & \textit{\textbf{.82}} & \textit{\textbf{.82}} & \textit{\textbf{.82}} & \textit{.68} & \textit{.68} & \textit{.68} & \textit{.80} & \textit{.80} & \textit{.80} & \textit{.73} & \textit{.73} & \textit{.73} \\
 &  & \textit{Macro-avg.} & \textit{.76} & \textit{\textbf{.84}} & \textit{.80} & \textit{\textbf{.82}} & \textit{.82} & \textit{\textbf{.82}} & \textit{.75} & \textit{.65} & \textit{.65} & \textit{.81} & \textit{.80} & \textit{.80} & \textit{.72} & \textit{.73} & \textit{.73} \\
\multicolumn{2}{r}{\multirow{2}{*}{\textit{Differences with the within-platform setting}}} & \textit{Micro-avg.} & \textit{-.18} & \textit{-.18} & \textit{-.18} & \textit{-.10} & \textit{-.10} & \textit{-.10} & \textit{-.14} & \textit{-.14} & \textit{-.14} & \multicolumn{3}{c}{\multirow{2}{*}{--}} & \multicolumn{3}{c}{\multirow{2}{*}{--}} \\
\multicolumn{2}{r}{} & \textit{Macro-avg.} & \textit{-.16} & \textit{-.08} & \textit{-.12} & \textit{-.10} & \textit{-.10} & \textit{-.10} & \textit{-.10} & \textit{-.16} & \textit{-.17} & \multicolumn{3}{c}{} & \multicolumn{3}{c}{} \\
\hline
\multirow{5}{*}{Cross-platform} & \multirow{5}{*}{Jira} & Negative & .84 & .51 & .63 & \textbf{.86} & .50 & .64 & .84 & .24 & .37 & .79 & \textbf{.77} & \textbf{.78} & .65 & .68 & .67 \\
 &  & Neutral & .59 & .96 & .73 & .62 & .95 & .75 & .51 & \textbf{.98} & .67 & .78 & .86 & \textbf{.82} & \textbf{.83} & .71 & .77 \\
 &  & Positive & \textbf{.93} & .45 & .61 & .91 & .57 & .70 & .92 & .35 & .51 & .86 & .76 & \textbf{.81} & .69 & \textbf{.81} & .75 \\
 &  & \textit{Micro-avg.} & \textit{.68} & \textit{.68} & \textit{.68} & \textit{.71} & \textit{.71} & \textit{.71} & \textit{.58} & \textit{.58} & \textit{.58} & \textit{\textbf{.80}} & \textit{\textbf{.80}} & \textit{\textbf{.80}} & \textit{.73} & \textit{.73} & \textit{.73} \\
 &  & \textit{Macro-avg.} & \textit{.79} & \textit{.64} & \textit{.66} & \textit{.79} & \textit{.67} & \textit{.69} & \textit{.76} & \textit{.52} & \textit{.52} & \textit{\textbf{.81}} & \textit{\textbf{.80}} & \textit{\textbf{.80}} & \textit{.72} & \textit{.73} & \textit{.73} \\
\multicolumn{2}{r}{\multirow{2}{*}{\textit{Differences with the within-platform setting}}} & \textit{Micro-avg.} & \textit{-.24} & \textit{-.24} & \textit{-.24} & \textit{-.21} & \textit{-.21} & \textit{-.21} & \textit{-.24} & \textit{-.24} & \textit{-.24} & \multicolumn{3}{c}{\multirow{2}{*}{\textit{--}}} & \multicolumn{3}{c}{\multirow{2}{*}{\textit{--}}} \\
\multicolumn{2}{r}{} & \textit{Macro-avg.} & \textit{-.13} & \textit{-.28} & \textit{-.26} & \textit{-.13} & \textit{-.25} & \textit{-.23} & \textit{-.09} & \textit{-.29} & \textit{-.30} & \multicolumn{3}{c}{} & \multicolumn{3}{c}{} \\ \hline
\multicolumn{18}{|c|}{\textit{Test set: Stack Overflow}} \\ \hline
\multirow{5}{*}{Within-platform} & \multirow{5}{*}{Stack Overflow} & Negative & .81 & .87 & .84 & \multicolumn{3}{c}{\multirow{5}{*}{--}} & .79 & .74 & .76 & .74 & .79 & .76 & .67 & .79 & .73 \\
 &  & Neutral & .86 & .81 & .84 & \multicolumn{3}{c}{} & .80 & .82 & .81 & .76 & .76 & .76 & .84 & .68 & .75 \\
 &  & Positive & .91 & .92 & .92 & \multicolumn{3}{c}{} & .88 & .90 & .89 & .89 & .84 & .86 & .85 & .90 & .87 \\
 &  & \textit{Micro-avg.} & \textit{.87} & \textit{.87} & \textit{.87} & \multicolumn{3}{c}{} & \textit{.83} & \textit{.83} & \textit{.83} & \textit{.80} & \textit{.80} & \textit{.80} & \textit{.79} & \textit{.79} & \textit{.79} \\
 &  & \textit{Macro-avg.} & \textit{.86} & \textit{.87} & \textit{.87} & \multicolumn{3}{c}{} & \textit{.82} & \textit{.82} & \textit{.82} & \textit{.80} & \textit{.80} & \textit{.79} & \textit{.79} & \textit{.79} & \textit{.78} \\
\hline
\multirow{5}{*}{Cross-platform} & \multirow{5}{*}{GitHub} & Negative & .71 & .72 & .72 & .71 & \textbf{.80} & .75 & .72 & .41 & .52 & \textbf{.74} & .79 & \textbf{.76} & .67 & .79 & .73 \\
 &  & Neutral & .71 & .80 & .75 & .79 & .75 & \textbf{.77} & .64 & \textbf{.88} & .74 & .76 & .76 & .76 & \textbf{.84} & .68 & .75 \\
 &  & Positive & \textbf{.92} & .78 & .84 & .90 & .85 & \textbf{.87} & .84 & .78 & .81 & .89 & .84 & .86 & .85 & \textbf{.90} & \textbf{.87} \\
 &  & \textit{Micro-avg.} & \textit{.77} & \textit{.77} & \textit{.77} & \textit{\textbf{.80}} & \textit{\textbf{.80}} & \textit{\textbf{.80}} & \textit{.72} & \textit{.72} & \textit{.72} & \textit{\textbf{.80}} & \textit{\textbf{.80}} & \textit{\textbf{.80}} & \textit{.79} & \textit{.79} & \textit{.79} \\
 &  & \textit{Macro-avg.} & \textit{.78} & \textit{.77} & \textit{.77} & \textit{\textbf{.80}} & \textit{\textbf{.80}} & \textit{\textbf{.80}} & \textit{.73} & \textit{.69} & \textit{.69} & \textit{\textbf{.80}} & \textit{\textbf{.80}} & \textit{.79} & \textit{.79} & \textit{.79} & \textit{.78} \\
\multicolumn{2}{r}{\multirow{2}{*}{\textit{Differences with the within-platform setting}}} & \textit{Micro-avg.} & \textit{-.10} & \textit{-.10} & \textit{-.10} & \textit{-.07} & \textit{-.07} & \textit{-.07} & \textit{-.11} & \textit{-.11} & \textit{-.11} & \multicolumn{3}{c}{\multirow{2}{*}{\textit{--}}} & \multicolumn{3}{c}{\multirow{2}{*}{\textit{--}}} \\
\multicolumn{2}{r}{} & \textit{Macro-avg.} & \textit{-.09} & \textit{-.10} & \textit{-.10} & \textit{-.06} & \textit{-.07} & \textit{-.07} & \textit{-.09} & \textit{-.13} & \textit{-.13} & \multicolumn{3}{c}{} & \multicolumn{3}{c}{} \\
\hline
\multirow{5}{*}{Cross-platform} & \multirow{5}{*}{Jira} & Negative & .77 & .34 & .48 & \textbf{.79} & .32 & .46 & .71 & .13 & .22 & .74 & \textbf{.79} & \textbf{.76} & .67 & \textbf{.79} & .73 \\
 &  & Neutral & .56 & .93 & .70 & .57 & .93 & .70 & .46 & \textbf{.97} & .62 & .76 & .76 & \textbf{.76} & \textbf{.84} & .68 & .75 \\
 &  & Positive & \textbf{.96} & .65 & .78 & .92 & .70 & .79 & \textbf{.96} & .38 & .54 & .89 & .84 & .86 & .85 & \textbf{.90} & \textbf{.87} \\
 &  & Micro-avg. & .68 & .68 & .68 & .68 & .68 & .68 & .54 & .54 & .54 & \textbf{.80} & .\textbf{80} & \textbf{.80} & \textbf{.79} & .79 & .79 \\
 &  & Macro-avg. & .76 & .64 & .65 & .76 & .65 & .65 & .71 & .49 & .46 & \textbf{.80} & \textbf{.80} & .79 & .79 & .79 & .78 \\
\multicolumn{2}{r}{\multirow{2}{*}{\textit{Differences with the within-platform setting}}} & \textit{Micro-avg.} & \textit{-.19} & \textit{-.19} & \textit{-.19} & \textit{-.19} & \textit{-.19} & \textit{-.19} & \textit{-.29} & \textit{-.29} & \textit{-.29} & \multicolumn{3}{c}{\multirow{2}{*}{\textit{--}}} & \multicolumn{3}{c}{\multirow{2}{*}{\textit{--}}} \\
\multicolumn{2}{r}{} & \textit{Macro-avg.} & \textit{-.10} & \textit{-.23} & \textit{-.22} & \textit{-.10} & \textit{-.22} & \textit{-.22} & \textit{-.11} & \textit{-.33} & \textit{-.36} & \multicolumn{3}{c}{} & \multicolumn{3}{c}{} \\ \hline
\multicolumn{18}{|c|}{\textit{Test set: Jira}} \\ \hline
\multirow{5}{*}{Within-platform} & \multirow{5}{*}{Jira} & Negative & .75 & .60 & .67 & \multicolumn{3}{c}{\multirow{5}{*}{--}} & .83 & .63 & .72 & .64 & .72 & .68 & .52 & .69 & .59 \\
 &  & Neutral & .87 & .89 & .88 & \multicolumn{3}{c}{} & .88 & .91 & .89 & .93 & .81 & .87 & .96 & .75 & .83 \\
 &  & Positive & .76 & .78 & .77 & \multicolumn{3}{c}{} & .79 & .81 & .80 & .69 & .93 & .79 & .63 & .90 & .74 \\
 &  & \textit{Micro-avg.} & \textit{.83} & \textit{.83} & \textit{.83} & \multicolumn{3}{c}{} & \textit{.86} & \textit{.86} & \textit{.86} & \textit{.82} & \textit{.82} & \textit{.82} & \textit{.77} & \textit{.77} & \textit{.77} \\
 &  & \textit{Macro-avg.} & \textit{.79} & \textit{.76} & \textit{.77} & \multicolumn{3}{c}{} & \textit{.83} & \textit{.78} & \textit{.80} & \textit{.75} & \textit{.82} & \textit{.78} & \textit{.69} & \textit{.78} & \textit{.72} \\
\hline
\multicolumn{1}{l}{\multirow{5}{*}{Cross-platform}} & \multicolumn{1}{c}{\multirow{5}{*}{GitHub}} & Negative & .57 & .64 & .61 & .57 & .61 & .59 & \textbf{.75} & .56 & .64 & .64 & \textbf{.72} & \textbf{.68} & .52 & .69 & .59 \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & Neutral & .89 & .79 & .84 & .88 & .80 & .84 & .90 & \textbf{.87} & \textbf{.88} & .93 & .81 & .87 & \textbf{.96} & .75 & .83 \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & Positive & .65 & .85 & .74 & .65 & .81 & .72 & \textbf{.71} & .91 & \textbf{.8} & .69 & \textbf{.93} & .79 & .63 & .9 & .74 \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \textit{Micro-avg.} & \textit{.78} & \textit{.78} & \textit{.78} & \textit{.78} & \textit{.78} & \textit{.78} & \textit{\textbf{.84}} & \textit{\textbf{.84}} & \textit{\textbf{.84}} & \textit{.82} & \textit{.82} & \textit{.82} & \textit{.77} & \textit{.77} & \textit{.77} \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \textit{Macro-avg.} & \textit{.70} & \textit{.76} & \textit{.73} & \textit{.70} & \textit{.74} & \textit{.71} & \textit{\textbf{.79}} & \textit{.78} & \textit{.77} & \textit{.75} & \textit{\textbf{.82}} & \textbf{\textit{.78}} & \textit{.69} & \textit{.78} & \textit{.72} \\
\multicolumn{2}{r}{\multirow{2}{*}{\textit{Difference with the within-platform setting}}} & \textit{Micro-avg.} & \textit{-.05} & \textit{-.05} & \textit{-.05} & \textit{-.05} & \textit{-.05} & \textit{-.05} & \textit{-.02} & \textit{-.02} & \textit{-.02} & \multicolumn{3}{c}{\multirow{2}{*}{\textit{--}}} & \multicolumn{3}{c}{\multirow{2}{*}{\textit{--}}} \\
\multicolumn{2}{r}{} & \textit{Macro-avg.} & \textit{-.09} & \textit{--} & \textit{-.04} & \textit{-.09} & \textit{-.02} & \textit{-.06} & \textit{-.04} & \textit{--} & \textit{-.03} & \multicolumn{3}{c}{} & \multicolumn{3}{c}{} \\
\hline
\multicolumn{1}{l}{\multirow{5}{*}{Cross-platform}} & \multicolumn{1}{l}{\multirow{5}{*}{Stack Overflow}} & Negative & .44 & .26 & .33 & .50 & .69 & .58 & .16 & .03 & .05 & \textbf{.64} & \textbf{.72} & \textbf{.68} & .52 & .69 & .59 \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & Neutral & .83 & .79 & .81 & .92 & .73 & .81 & .75 & \textbf{.94} & .83 & .93 & .81 & \textbf{.87} & \textbf{.96} & .75 & .83 \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & Positive & .57 & .85 & .68 & .63 & .90 & .74 & .72 & .49 & .58 & \textbf{.69} & \textbf{.93} & \textbf{.79} & .63 & .90 & .74 \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \textit{Micro-avg.} & \textit{.73} & \textit{.73} & \textit{.73} & \textit{.76} & \textit{.76} & \textit{.76} & \textit{.73} & \textit{.73} & \textit{.73} & \textit{\textbf{.82}} & \textit{\textbf{.82}} & \textit{\textbf{.82}} & \textit{.77} & \textit{.77} & \textit{.77} \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \textit{Macro-avg.} & \textit{.62} & \textit{.63} & \textit{.61} & \textit{.68} & \textit{.78} & \textit{.71} & \textit{.54} & \textit{.49} & \textit{.49} & \textit{\textbf{.75}} & \textit{\textbf{.82}} & \textit{\textbf{.78}} & \textit{.69} & \textit{.78} & \textit{.72} \\
\multicolumn{2}{r}{\multirow{2}{*}{\textit{Differences with the within-platform setting}}} & \textit{Micro-avg.} & \textit{-.10} & \textit{-.10} & \textit{-.10} & \textit{-.07} & \textit{-.07} & \textit{-.07} & \textit{-.13} & \textit{-.13} & \textit{-.13} & \multicolumn{3}{c}{\multirow{2}{*}{--}} & \multicolumn{3}{c}{\multirow{2}{*}{--}} \\
\multicolumn{2}{r}{} & \textit{Macro-avg.} & \textit{-.17} & \textit{-.13} & \textit{-.16} & \textit{-.11} & \textit{+.02} & \textit{-.06} & \textit{-.29} & \textit{-.29} & \textit{-.31} & \multicolumn{3}{c}{} & \multicolumn{3}{c}{} \\ %\cline{3-12}
\hline
\end{tabular}%
}
\end{table*}
